Stability and performance in transient average constrained economic MPC without terminal constraints

In this paper, we investigate system theoretic properties of transient average constrained economic model predictive control (MPC) without terminal constraints. We show that the optimal open-loop solution passes by the optimal steady-state for consecutive time instants. Using this turnpike property and suitable controllability conditions, we provide closed-loop performance bounds. Furthermore, stability is proved by combining the rotated value function with an input-to-state (ISS) Lyapunov function of an extended state related to the transient average constraints. The results are illustrated with a numerical example.

==> backup_traj_conv.tex <==
\begin{theo}
	Assume furthermore that there exists a function $\eta\in\mathcal{L}_{\mathbb{N}}$ such that for $N\geq N_3$ it holds $\tilde{J}^\ast_N(x,H)\geq N\alpha(\norm{x-x_s}+\Hnorm)$ for all $x\in\mathbb{X}\setminus x_s$ and $H\in\mathbb{H}\setminus H^s$ for which $\norm{x-x_s}+\Hnorm >\eta(N)$ with some $\alpha\in\mathcal{K}_\infty$. Then there exists $\tilde{N}_6$ and $\tilde{\sigma}_c\in\mathcal{L}_{\mathbb{N}}$ such that for all $(x,H)\in\mathbb{X}\times\mathbb{H}$, $N\geq \tilde{N}_6+1 $ and all $k\geq N$ it holds
	\begin{equation}\label{eq:traj_conv_ass1}
	\begin{split}
	&\norm{x_{\mu_N}(k,x)-x_s}+\HnormB{H^{\mathrm{cl}}(k)}\\\leq &\max \{  \eta(N), \, \alpha^{-1}(\tilde{ \sigma}_c (N-\tilde{N}_6))\}.
	\end{split}
	\end{equation}
	
	Moreover, if for all $N\geq \tilde{N}_6$ it holds $\tilde{J}^\ast_N(x,H)\leq N\tilde{ l}(x_s,u_s)+ N\bar{\alpha}(\norm{x-x_s}+\Hnorm)$ for some $\bar{\alpha}\in\mathcal{K}_\infty$, then for all $N\geq \tilde{N}_6$ it holds for all $k\in\mathbb{I}_{[1,N-1]}$ and any $(x,H)\in\mathbb{X}\times \mathbb{H}$
	\begin{equation}\label{eq:traj_conv_ass2}
	\begin{split}
	&\norm{x_{\mu_N}(k,x)-x_s}+\HnormB{H^{\mathrm{cl}}(k)}\\\leq &\max \{  \eta(N), \, \alpha^{-1}(\bar{\alpha}(\norm{x-x_s}+\Hnorm)+\tilde{\sigma}_c (N-\tilde{N}_6))\}.
	\end{split}
	\end{equation}
\end{theo}

\begin{proof}
	\textit{Part II: Showing~\eqref{eq:traj_conv_ass1} and~\eqref{eq:traj_conv_ass2}}.
	In the following we will make use of the estimate
	\begin{equation}\label{eq:proof_traj_conv_estimate_residuum}
	\begin{split}
	\tilde{J}_K^{\mathrm{cl}} (x,H,\mu_N)\leq &\tilde{J}_N^\ast (x,H)-\tilde{J}^\ast_N (x_{\mu_N}(K),H^{\mathrm{cl}}(K))\\&+\sigma_R (N_R)+K\sigma_c(N-N_c)+\tau\overline{\vartheta}_h
	\end{split}
	\end{equation} with $\sigma_R,\,\sigma_c\in\mathcal{L}_{\mathbb{N}}$ where $N_R:=N-N_2-(4T+1)(T-1)-1$, $N_c:=N-N_2-T^2-1$ and $\tau:=\min\{K,T-1\}$ which holds for all $(x,H)\in\mathbb{X}\times \mathbb{H}$ and $N\geq \tilde{N}_6:=\max \{ N_2+\frac{4T\hat{C}'}{\rho(\epsilon)}+(4T+1)(T-1)+1,N_3+1 \}$ with $\epsilon\leq \bar{\epsilon}$. For clarity, we refer for the proof of this to~\cite[Thm. x]{SA}. As one can find there, it holds $\sigma_R (N_R)=\sigma'_R (\tilde{\sigma}_{c,1}(N_R))$ with $\sigma'_R(\epsilon)=12 \gamma_v ((1+2pL_h)\epsilon)+6(\alpha_\lambda(\epsilon)+(T-1)2L_h \norm{\bl}\epsilon)$ and $\tilde{\sigma}_{c,1}(N_R)=\rho^{-1}(\frac{4 T \hat{C}'}{N_R})$. However, we remark that~\eqref{eq:proof_traj_conv_estimate_residuum} is shown by ensuring that there exists $k_x\in\mathcal{T}^{'\epsilon}_{[T-1,N-N_2]} ((u^\ast_{N,x_i,H^i},x_i), (\tilde{u}^\ast_{N,x_i,H^i},x_i)$ with $x_i=\{x,x_{\mu_N}(K)\}$ and $H^i=\{H,H^{\mathrm{cl}}(K) \}$ as well as using Lemma~\ref{lem:residuum}. 
	
	Now, we suppose that $\norm{x_{\mu_N}(k)-x_s}+\HnormB{H^{\mathrm{cl}}(k)}> \eta(N)$ and use~\eqref{eq:proof_traj_conv_estimate_residuum} with $K=N$, $x_{\mu_N}(k-N)$ and $H^{\mathrm{cl}}(k_N)$. Combining this with $N\alpha(\norm{x-x_s}+\Hnorm)\leq \tilde{J}^\ast_N(x,H)$ yields $\alpha(\norm{x_{\mu_N}(k)-x_s}+\HnormB{H^{\mathrm{cl}}(k)})\leq \sigma_c (N_c)+\frac{1}{N}\sigma_R (N_R)+\frac{\tau}{N}\overline{\vartheta}_h$. Furthermore, due to our choice of $\tilde{N}_6$ and since $N\geq \tilde{N}_6+1$, we obtain $\sigma_c (N_c)+\frac{1}{N}\sigma_R (N_R)+\frac{\tau}{N}\overline{\vartheta}_h\leq \sigma_c(N-\tilde{N}_6)+\frac{1}{N-\tilde{N}_6}\sigma_R (N-\tilde{N}_6)+\frac{\tau}{N-\tilde{N}_6}\overline{\vartheta}_h=:\tilde{\sigma}_c (N-\tilde{N}_6)$ with $\tilde{\sigma}_c\in\mathcal{L}_{\mathbb{N}}$ which yields $\norm{x(k)-x_s}+\HnormB{H^{\mathrm{cl}}(k)}\leq \alpha^{-1} (\tilde{\sigma}_c (N-\tilde{N}_6))$. Combining this with the case $\norm{x_{\mu_N}(k)-x_s}+\HnormB{H^{\mathrm{cl}}(k)}\leq \eta(N)$ it follows assertion~\eqref{eq:traj_conv_ass1}.
	
	Again, we suppose that $\norm{x_{\mu_N}(k)-x_s}+\HnormB{H^{\mathrm{cl}}(k)}> \eta(N)$ holds and make use of~\eqref{eq:proof_traj_conv_estimate_residuum} but this time with $K=k\leq N$. Combining $0\leq \tilde{J}^\ast_k(x,H)\leq \tilde{J}^{\mathrm{cl}}_k (x,H,\mu_N)$ with the conditions of Thm.~\ref{thm:performance} yields $N\alpha(\norm{x_{\mu_N}(k)-x_s}+\HnormB{H^{\mathrm{cl}}(k)})\leq N\bar{\alpha} (\norm{x-x_s}+\Hnorm)+\sigma_R(N_R)+k\sigma_c(N_c)+ \tau\overline{\vartheta}_h$. Rearranging this, using the definition of $\tilde{\sigma_c}(N-\tilde{N}_6)$ and considering the case $\norm{x_{\mu_N}(k)-x_s}+\HnormB{H^{\mathrm{cl}}(k)}\leq \eta(N)$ then yields assertion~\eqref{eq:traj_conv_ass2}.
\end{proof}
